Lipschitz Bandits with Batched Feedback

In this paper, we study Lipschitz bandit problems with batched feedback, where the expected reward is Lipschitz and the reward observations are communicated to the player in batches. We introduce a novel landscape-aware algorithm, called Batched Lipschitz Narrowing (BLiN), that optimally solves this problem. Specifically, we show that for a $T$-step problem with Lipschitz reward of zooming dimension $d_z$, our algorithm achieves theoretically optimal (up to logarithmic factors) regret rate $\widetilde{\mathcal{O}}\left(T^{\frac{d_z+1}{d_z+2}}\right)$ using only $ \mathcal{O} \left( \log\log T\right) $ batches. We also provide complexity analysis for this problem. Our theoretical lower bound implies that $\Omega(\log\log T)$ batches are necessary for any algorithm to achieve the optimal regret. Thus, BLiN achieves optimal regret rate (up to logarithmic factors) using minimal communication.

==> tex/lower-bound-dz-static.tex <==
% \begin{proof}[Proof of Theorem \ref{thm:lower-static-dz}]
    Fixing $k$ and $1\leq i\leq M_k$, we show that $\mu_{k,i}$ is $1$-Lipschitz and the zooming dimension equals to $d_z$.
    
    Firstly, for any $(\alpha_1,\beta_1)$ and $(\alpha_2,\beta_2)$, we have
    \begin{align*}
        &\mu_{k,i}((\alpha_1,\beta_1))-\mu_{k,i}((\alpha_2,\beta_2))\\
        \leq&\mu_{k,i}((\alpha_1,\beta_1))-\mu_{k,i}((\alpha_1,\beta_2))\\
        &+\mu_{k,i}((\alpha_1,\beta_2))-\mu_{k,i}((\alpha_2,\beta_2))\\
        \leq&\frac{1}{2}\|\beta_1-\beta_2\|_\infty+\frac{1}{2}\big(\nu_{k,i}((\alpha_1,0_{d-d_z}))-\nu_{k,i}((\alpha_2,0_{d-d_z}))\big)\\
        \leq&\frac{1}{2}(\|\beta_1-\beta_2\|_\infty+\|\alpha_1-\alpha_2\|_\infty)\\
        \leq&\|(\alpha_1-\alpha_2,\beta_1-\beta_2)\|_\infty.
    \end{align*}
    Therefore, $\mu_{k,i}$ is $1$-Lipschitz.

    Secondly, for any $r\geq r_k$, (\ref{eq:constuct3-dz}) yields that $S(16r)=[0,1]^{d_z}\times[0, 32r]^{d-d_z}$. Therefore, we have $N_r=32^{d-d_z}r^{-d_z}$, and the zooming dimension equals to $d_z$.

    Then we show that an argument similar to Theorem \ref{st_lb} yields the lower bound we need. Recall that each $u_{k,i}$ is in $\A_{d_z}$. For convenience, we write $u_{k,i}=(\hat{u}_{k,i},0_{d-d_z})$. Let $H_{k,i}=\B_{d_z}(\hat{u}_{k,i},\frac{3}{8}r_k)\times[0,1]^{d-d_z}$, where $\B_{d_z}(\hat{u}_{k,i},\frac{3}{8}r_k)$ denotes the $d_z$-dimensional ball with center $\hat{u}_{k,i}$ and radius $\frac{3}{8}r_k$. It is easy to verify the following properties of construction (\ref{eq:constuct1-dz}),(\ref{eq:constuct2-dz}) and (\ref{eq:constuct3-dz}):
    \begin{enumerate}
        \item For any $2\leq i\leq M_k$, $\mu_{k,i}(z)=\mu_{k,1}(z)$ for any $z\in\mathcal{A}\setminus H_{k,i}$;
        \item For any $2\leq i\leq M_k$, $\mu_{k,1}(z)\leq\mu_{k,i}(z)\leq\mu_{k,1}(z)+\frac{r_k}{4}$, for any $z\in H_{k,i}$;
        \item For any $1\leq i\leq M_k$, under $I_{k,i}$, pulling an arm that is not in $H_{k,i}$ incurs a regret at least $\frac{r_k}{16}$. 
    \end{enumerate}
    
    
    
%     The lower bound of expected regret relies on the following lemma.
%     \begin{lemma}\label{lem:kld-dz}
%     	For any policy $\pi$, there exists a problem instance $I\in\mathcal{I}_k$ such that
%     	\begin{equation*}
%     	    \E \[ R_T(\pi) \] \geq  \frac{r_k}{64}\cdot\sum_{j=1}^B \( t_j-t_{j-1} \) \exp\left\{-\frac{t_{j-1}r_k^2}{32(M_k-1)}\right\}.
%     	\end{equation*}
    	 
%     % 	\textcolor{red}{check the constants}
%     \end{lemma} 

%     \begin{proof}
%         % Let $S_{k,i}=\B(u_{k,i},\frac{3}{8}r_k)$ (the ball with center $u_{k,i}$ and radius $\frac{3}{8}r_k$). It is easy to verify the following properties of construction (\ref{eq:constuct1}) and (\ref{eq:constuct2}):
%         % \begin{enumerate}
%         %     \item For any $2\leq i\leq M_k$, $\mu_{k,i}(x)=\mu_{k,1}(x)$ for any $x\in\mathcal{A}-S_{k,i}$;
%         %     \item For any $2\leq i\leq M_k$, $\mu_{k,1}(x)\leq\mu_{k,i}(x)\leq\mu_{k,1}(x)+\frac{r_k}{4}$, for any $x\in S_{k,i}$;
%         %     \item For any $1\leq i\leq M_k$, under $I_{k,i}$, pulling an arm that is not in $S_{k,i}$ incurs a regret at least $\frac{r_k}{8}$. 
%         % \end{enumerate}
        
%         Let $ x_t $ denote the choices of policy $\pi$ at time $t$, and $y_t$ denote the reward. Additionally, for $t_{j-1}<t\leq t_j$, we define $\Pr_{k.i}^t$ as the distribution of sequence $\left(x_1,y_1,\cdots,x_{t_{j-1}},y_{t_{j-1}}\right)$ under instance $I_{k,i}$ and policy $\pi$. It holds that 
%         \begin{align} 
%             \sup_{I\in\mathcal{I}_k} \E R_T(\pi)  
%             \geq&
%             \frac{1}{M_k}\sum_{i=1}^{M_k} \E_{\Pr_{k,i}} \left[ R_T(\pi) \right] \nonumber \\
%             \geq&
%             \frac{1}{M_k}\sum_{i=1}^{M_k} \sum_{t=1}^T\E_{\Pr_{k,i}^t} \left[ R^t(\pi) \right] \nonumber \\
%             \geq&
%             \frac{r_k}{16}\sum_{t=1}^T\frac{1}{M_k}\sum_{i=1}^{M_k} \Pr_{k,i}^t(x_t\notin H_{k,i}),\label{eq:spl-dz}
%         \end{align} 
%         where $R^t(\pi)$ denotes the regret incurred by policy $\pi$ at time $t$. 
            
%         From our construction, it is easy to see that $H_{k,j}\cap H_{k,j}=\varnothing$, so we can construct a test $\Psi$ such that $x_t\in H_{k,i}$ implies $\Psi= i$.  
%         % \textcolor{red}{(ZF: it should be ``$x_t\in S_i$ implies $\Psi= i$'' ?)}. 
%         Then from Lemma \ref{lem:test-tree}, 
%         \begin{align*}
%             & \; \frac{1}{M_k}\sum_{i=1}^{M_k} \Pr_{k,i}^t(x_t\notin H_{k,i}) \\ 
%             \geq& \;  
%             \frac{1}{M_k}\sum_{i=1}^{M_k} \Pr_{k,i}^t(\Psi\neq i) \\
%             \geq& \;  
%             \frac{1}{2M_k}\sum_{i=2}^{M_k} \exp 
%             \left\{-D_{KL}\left(\Pr_{k,1}^t\|\Pr_{k,i}^t\right)\right\}.
%         \end{align*} 
%         % Now we calculate $D_{KL}\left(\Pr_1^t\|\Pr_i^t\right)$. For convenience, assume that sequence $\left(x_1,r_1,\cdots,x_{t_{j-1}},r_{t_{j-1}}\right)$ obeys distribution $\Pr_1^t$, and $\left(\wt{x}_1,\wt{r}_1,\cdots,\wt{x}_{t_{j-1}},\wt{r}_{t_{j-1}}\right)$ obeys distribution $\Pr_i^t$. Then from the chain rule of KL-Divergence, we have

%         To avoid notational clutter, for any $s,s'$ ($s \ge s'$), define 
%         \begin{align*}
%             (\x, \y )_{:s}^{:s'} =& \; (x_1, y_1,\cdots,x_{s'}, y_{s'}, \cdots ,x_s) . 
%             % \y_{:s} =& \; (y_1,y_2,\cdots,y_s) .
%         \end{align*}
        
%         Now we calculate $D_{KL}\left(\Pr_{k,1}^t\|\Pr_{k,i}^t\right)$. From the chain rule of KL-Divergence, we have
%         \begin{align}
%             & \; D_{KL}\left(\Pr_{k,1}^t\|\Pr_{k,i}^t\right) \nonumber \\
%             =& \;
%             D_{KL}\left(\Pr_{k,1}^t \( (\x ,\y)_{:t_{j-1}}^{:t_{j-1}} \) \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}}^{:t_{j-1}} \) \right)\nonumber\\
%             =& \;
%             D_{KL}\left(\Pr_{k,1}^t \(  (\x ,\y)_{:t_{j-1}}^{:t_{j-1} - 1} \)  \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}}^{:t_{j-1} - 1} \) \right)\nonumber\\ 
%             % &+\E_{\Pr_{k,1}}\left(D_{KL}\left(\Pr_{k,1}^t(y_{t_{j-1}}| (\x ,\y)_{:t_{j-1}}^{:t_{j-1} - 1} ) \| \Pr_{k,i}^t(y_{t_{j-1}}| (\x ,\y)_{:t_{j-1}}^{:t_{j-1} - 1} )\right)\right)\nonumber\\ 
%             % \leq& \; 
%             % D_{KL}\left(\Pr_{k,1}^t(x_1,y_1,\cdots,x_{t_{j-1}-1},y_{t_{j-1}-1}) \| \Pr_{k,i}^t(x_1,y_1,\cdots,x_{t_{j-1}-1},y_{t_{j-1}-1})\right)\nonumber\\
%             &+\E_{\Pr_{k,1}}\left(D_{KL}\left(\Pr_{k,1}^t(y_{t_{j-1}}|x_{t_{j-1}}) \| \Pr_{k,i}^t(y_{t_{j-1}}|x_{t_{j-1}})\right)\right) \label{chain_eq1-dz}\\
%             \le& \;
%             D_{KL}\left(\Pr_{k,1}^t \(  (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \)  \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \) \right)\nonumber\\ 
%             &+\E_{\Pr_{k,1}}\left(D_{KL}\left(\Pr_{k,1}^t(y_{t_{j-1}}|x_{t_{j-1}}) \| \Pr_{k,i}^t(y_{t_{j-1}}|x_{t_{j-1}})\right)\right) \label{chain_eq1.5-dz}\\
%             \leq& \;
%             D_{KL}\left(\Pr_{k,1}^t\( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \) \| \Pr_{k,i}^t\( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \)\right)\nonumber\\
%             &+\E_{\Pr_{k,1}}\left(D_{KL}\left(N(\mu_{k,1}(x_{t_{j-1}}),1) \| N(\mu_{k,i}(x_{t_{j-1}}),1)\right)\right) \label{chain_eq2-dz}\\
%             =& \;
%             D_{KL}\left(\Pr_{k,1}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \) \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \)\right)\nonumber\\ 
%             &+\E_{\Pr_{k,1}}\left(\frac{1}{2}\left(\mu_{k,1}(x_{t_{j-1}})-\mu_{k,i}(x_{t_{j-1}})\right)^2\right) \nonumber\\
%             \leq& \;
%             D_{KL}\left(\Pr_{k,1}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \) \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \)\right)\nonumber\\
%             &+\E_{\Pr_{k,1}}\left(\bm{1}_{\{x_{t_{j-1}}\in S_{k,i}\}}\cdot\frac{1}{2}\left(\frac{r_k}{4}\right)^2\right)\label{chain_use_prop-dz}\\
%             =& \;
%             D_{KL}\left(\Pr_{k,1}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \) \| \Pr_{k,i}^t \( (\x ,\y)_{:t_{j-1}-1}^{:t_{j-1} - 1} \)\right)\nonumber\\
%             &+\frac{r_k^2}{32}\cdot\Pr_{k,1}\left(x_{t_{j-1}}\in S_{k,i}\right),\label{chain_singal-dz}
%         \end{align}
%         where (\ref{chain_eq1-dz}) uses chain rule for KL-divergence and the conditional independence of the reward, (\ref{chain_eq1.5-dz}) removes dependence on $x_{t_{j - 1}}$ in the first term by another use of chain rule and nonnegativity of KL-divergence, (\ref{chain_eq2-dz}) uses that the rewards are corrupted by a standard normal noise, and (\ref{chain_use_prop-dz}) uses the first two properties of the construction.
        
%         Since (\ref{chain_singal-dz}) holds for all $t \le t_{j-1}$, we conclude that
%         % then decompose the KL-Divergence step by step and conclude that
%         \begin{align}\label{chain-dz}
%             D_{KL}\left(\Pr_{k,1}^t\|\Pr_{k,i}^t\right)\leq\frac{r_k^2}{32}\sum_{s\leq t_{j-1}}\Pr_{k,1}\left(x_s\in H_{k,i}\right)=\frac{r_k^2}{32} \E_{\Pr_{k,1}}\tau_i,
%         \end{align}
%         where $\tau_i$ denotes the number of pulls of arms in $H_{k,i}$ before the batch containing $t$. Then for all $t \in ( t_{j-1}, t_j]$, we have  
%         \begin{align}
%             & \; \frac{1}{M_k}\sum_{i=1}^{M_k} \Pr_{k,i}^t(x_t\notin H_{k,i}) \nonumber \\
%             \geq& \; 
%             \frac{1}{2M_k}\sum_{i=2}^{M_k} \exp\left\{-\frac{r_k^2}{32} \E_{\Pr_{k,1}}\tau_i\right\} \nonumber \\ 
%             \geq& \;  
%             \frac{M_k-1}{2M_k}\exp\left\{-\frac{r_k^2}{32(M_k-1)}\sum_{i=2}^{M_k}\E_{\Pr_{k,1}} \tau_i \right\} \label{eq:use-jensen-dz}  \\
%             \geq& \; 
%             \frac{1}{4}\exp\left\{-\frac{r_k^2t_{j-1}}{32(M_k-1)}\right\}, \label{eq:hyp-dz}
%         \end{align} 
%         where (\ref{eq:use-jensen-dz}) uses the Jensen' inequality, and (\ref{eq:hyp-dz}) uses the fact that $\sum_{i=2}^{M_k}\tau_i\leq t_{j-1}$. Finally, we substitute (\ref{eq:hyp-dz}) to (\ref{eq:spl-dz}) to finish the proof. 
%     \end{proof} 
    
% 	Since $M_k=t_{k-1}r_k^2$, the expected regret of policy $\pi$ satisfies
% 	\begin{align*} 
% 		\E \[ R_T(\pi) \] 
% 		&\geq 
% 		\frac{r_k}{64} \cdot\sum_{j=1}^B \( t_j-t_{j-1} \) \exp\left\{-\frac{t_{j-1}r_k^2}{32(M_k-1)}\right\}\\ 
% 		&\geq
% 		\frac{r_k}{64} \cdot\sum_{j=1}^B \( t_j-t_{j-1} \) \exp\left\{-\frac{t_{j-1}r_k^2}{16M_k}\right\}\\
% 		&\geq 
% 		\frac{r_k}{64} \cdot\sum_{j=1}^B \( t_j-t_{j-1}\) \exp\left\{-\frac{t_{j-1}}{16t_{k-1}}\right\}
% 	\end{align*}
% 	on an instance $I_{k,i}\in\I_k$.
	
% 	By omitting terms with $j > k$ in the above summation, we have 
% 	\begin{align*}
% 	    \E[R_T(\pi)]&\geq\frac{r_k}{64} \cdot \sum_{j=1}^B \( t_j-t_{j-1}\) \exp\left\{-\frac{t_{j-1}}{16t_{k-1}}\right\}  \\
% 	    &\ge 
% 	    \frac{r_k}{64} \cdot \sum_{j=1}^{k} \( t_j-t_{j-1}\) \exp\left\{-\frac{1}{16}\right\} \\
% 	    &= \frac{1}{64e^\frac{1}{16}}r_kt_k\\
% 		&= \frac{1}{64e^\frac{1}{16}}\cdot\frac{t_k}{t_{k-1}^\frac{1}{d_z+2}}.
% 	\end{align*}
%    	The above analysis can be applied for any $k>1$. For the first batch $(0, t_1]$, we can easily construct a set of instances where the worst-case regret is at least $t_1$, since no information is available during this time.  Thus, there exists a problem instance such that
%    	\begin{align*}
%    	    \E[R_T(\pi)]\geq\frac{1}{64e^\frac{1}{16}}\max\left\{t_1,\frac{t_2}{t_1^\frac{1}{d_z+2}},\cdots,\frac{t_B}{t_{B-1}^\frac{1}{d_z+2}}\right\}.
%    	\end{align*}
    
%     Since $0<t_1<\cdots<t_B=T$, we further have
%     \begin{align*}
%         &\max\left\{t_1,\frac{t_2}{t_1^\varepsilon},\cdots,\frac{t_B}{t_{B-1}^\varepsilon}\right\}\\
%         \geq&\left(t_1^{\varepsilon^{B-1}}\cdot\left(\frac{t_2}{t_1^\varepsilon}\right)^{\varepsilon^{B-2}}\cdots\left(\frac{t_{B-1}}{t_{B-2}}^\varepsilon\right)^{\varepsilon}\cdot\frac{t_B}{t_{B-1}^\varepsilon}\right)^{\frac{1}{\sum_{i=1}^{B-1}}\varepsilon^i}\\
%         =&T^{\frac{1-\varepsilon}{1-\varepsilon^B}},
%     \end{align*}
%     where $\varepsilon=\frac{1}{d_z+2}$. Combining the above two inequalities, we conclude that
%     % \begin{align*}
%     %     % &\max\left\{t_1,\frac{t_2}{t_1^\varepsilon,\cdots,\frac{t_B}{t_{B-1}^\varepsilon\right\}\\
%     %     % \geq&$\left(t_1^{\varepsilon^{B-1}}\cdot\left(\frac{t_2}{t_1^\varepsilon}\right)^{\varepsilon^{B-2}}\cdots\frac{t_B}{t_{B-1}^\varepsilon}\right)
%     % \end{align*}
    
%    	\begin{equation*}
% 	    \E \[ R_T(\pi) \]
% 	    \geq
% 	    \frac{1}{64e^\frac{1}{16}}\cdot T^{\frac{1-\frac{1}{d_z+2}}{1-\left(\frac{1}{d_z+2}\right)^B}}. \qedhere
% 	\end{equation*}
    
% 	% Since $N_r\leq r^{-d}$ holds for all instances,
% 	% \begin{align*}
% 	%     \sum_{r=2^{-i},\; r\geq r_0}\frac{N_r}{r}\log T\leq2r_0^{-d-1}\log T.
% 	% \end{align*} 
% 	% Then we have
% 	% \begin{align}
%  %    	\begin{split}	
%  %    	    R_z(T)=&\inf_{r_0}\left\{r_0T+\sum_{r=2^{-i},\;r\geq r_0}\frac{N_r}{r}\log T\right\}\\
%  %    		\leq&
%  %    		\inf_{r_0}\left\{r_0T+\frac{2}{r_0^{d+1}}\log T\right\}\\
%  %    		\leq&
%  %    		2(\log T)^{\frac{1}{d+2}}T^{1-\frac{1}{d+2}}.
%  %        \end{split}\label{ineq:rzt}
%  %    \end{align}
%  %    As a consequence, for instance $I$ satisfying (\ref{lower_real}),
%  %    \begin{align*}
%  %        &\; \E[R_T(\pi)] \\ 
%  %        \geq& \; 
%  %        \frac{1}{32e^\frac{1}{16}}\left(\frac{1}{2(\log T)^\frac{1}{d+2}}\right)^\frac{1}{1-\left(\frac{1}{d+2}\right)^B}\cdot R_z(T)^\frac{1}{1-\left(\frac{1}{d+2}\right)^B}\\
%  %        \geq& \; 
%  %        \frac{1}{32e^\frac{1}{16}\cdot2^\frac{1}{1-\frac{1}{d+2}}}\cdot(\log T)^{-\frac{\frac{1}{d+2}}{1-\left(\frac{1}{d+2}\right)^B}}\cdot R_z(T)^\frac{1}{1-\left(\frac{1}{d+2}\right)^B}\\
%  %        \geq& \; 
%  %        \frac{1}{128e^\frac{1}{16}}\cdot(\log T)^{-\frac{\frac{1}{d+2}}{1-\left(\frac{1}{d+2}\right)^B}}\cdot R_z(T)^\frac{1}{1-\left(\frac{1}{d+2}\right)^B}, 
%  %    \end{align*}
%  %    which finishes the proof. 
%     % Hence, the proof is completed.
% \end{proof} 

Now we combine all techniques in above analysis to obtain the lower bound for general $d_z$ and adaptive grid, and thus proves \textcolor{red}{Theorem}.

\begin{theorem}
    \label{thm:lower-adaptive-dz}
    Consider Lipschitz bandit problems with ambient dimension $d$ and time horizon $T$ such that the grid of reward communication $\mathcal{T}$ is adaptively determined by the player. If $B$ rounds of communications are allowed, then for any policy $\pi$ and any $d_z\leq d$, there exists an instance with zooming dimension $d_z$ such that 
	\begin{align*} 
	    \E \left[ R_T(\pi) \right] 
	    \geq \frac{1}{512B^2}T^{\frac{1-\frac{1}{d_z+2}}{1-\left(\frac{1}{d_z+2}\right)^B}}.
	\end{align*}
\end{theorem}

\begin{proof}[Proof of Theorem \ref{thm:lower-adaptive-dz}]
    %   \TW{Very nice explanation. You can place the above two paragraphs between the theorem statement and the proof, and the proof starts from "Firstly, we define... ". } 
    
    % an instance in world $\mathcal{I}_j$ such that the regret of the policy is not less than $r_jT_j$, which gives the lower bound we need.}
    The main argument in the proof of Theorem \ref{thm:lower-adaptive-dz} is similar to that of Theorem \ref{thm:ada_lb}. To construct hard instances in the $d$-dimensional space, we use the `linear-decaying extension' technique, which is the same as the proof of Theorem \ref{thm:lower-static-dz}.
    
    Firstly, we define $r_j=\frac{1}{T_{j-1}^\varepsilon B}$ and $M_j=\frac{1}{r_j^{d_z}}$, where $\varepsilon=\frac{1}{d_z+2}$.
    % \begin{align*}
    %     r_j=\frac{1}{T_{j-1}^\varepsilon B} = T^{\frac{-\varepsilon(1-\varepsilon^{j-1})}{1-\varepsilon^B}}/B\quad\text{and}\quad M_j=\frac{1}{r_j^d}. 
    % \end{align*} 
    From the definition, we have
    \begin{align} 
        T_{j-1}r_j^2=\frac{1}{r_j^{d_z} B^2}=\frac{M_j}{B^2}. \label{eq:rm-relation-dz}
    \end{align}
    For $1\leq j\leq B$, we can find sets of arms $\mathcal{U}_j=\{u_{j,1},\cdots,u_{j,M_j}\}\in\mathcal{A}_{d_z}$ such that (a) $d_{\mathcal{A}}(u_{j,m},u_{j,n})\geq r_j$ for any $m\neq n$, and (b) $u_{1,M_1}=\cdots=u_{B,M_B}$. 
    % \TW{add: we can always find such $\mathcal{U}_j$ since its cardinality is smaller than the packing number. or similar comment.  }
    
    Then we present the construction of worlds $\mathcal{I}_1,\cdots,\mathcal{I}_B$. For $1\leq j\leq B-1$, we let $\I_{j}=\{\I_{j,k}\}_{k=1}^{M_j-1}$. We first construct a set of expected reward functions $\{\nu_{j,1},\cdots,\nu_{j, M_j-1}\}$ on $\mathcal{A}_{d_z}$. For each $1\leq k\leq M_j-1$, we define $\nu_{j,k}$ as
    \begin{align}
    	\nu_{j,k}(z)=
    	\begin{cases}
    		\frac{r_1}{2}+\frac{r_j}{16}+\frac{r_B}{16},\;\text{if}\;z=u_{j,k},\\
    		\frac{r_1}{2}+\frac{r_B}{16},\;\text{if}\;z=u_{j,M_j},\\
                \max\left\{\frac{r_1}{2},\max_{u\in\mathcal{U}_j}\left\{\nu_{j,k}(u)-d_\mathcal{A}(z,u)\right\}\right\},\\
                \quad\text{if}\;z\in\A_{d_z}\setminus\mathcal{U}_j.
    	\end{cases} \label{eq:instance-ada1-dz-nu}
    \end{align}
    Based on $\{\nu_{j,k}\}_{k=1}^{M_j-1}$, the expected reward of $I_{j,k}$ is defined as
    \begin{align}\label{eq:instance-ada1-dz-mu}
    	\mu_{j,k}((\alpha,\beta))=\frac{1}{2}\left(\nu_{j,k}((\alpha,0_{d-d_z}))-\|\beta\|_\infty\right),
    \end{align}
    where $(\alpha,\beta)$ is the concatenation of $\alpha\in[0,1]^{d_z}$ and $\beta\in[0,1]^{d-d_z}$. For $j=B$, we let $\I_B=\{I_{B}\}$. We first define a function $\nu_B$ on $\A_{d_z}$ as
    \begin{align}
    	\nu_{B}(z)=
    	\begin{cases}
    		\frac{r_1}{2}+\frac{r_B}{16},\;\text{if}\;z=u_{B, M_B},\\
                \max\left\{\frac{r_1}{2},\max_{u\in\mathcal{U}_j}\left\{\mu_{j,k}(u)-d_\mathcal{A}(z,u)\right\}\right\},\\
                \quad\text{if}\;z\in\A_{d_z}/\{u_{B,M_B}\}.
    	\end{cases} \label{eq:instance-ada2-dz-nu}
    \end{align}
    Then the expected reward of $I_B$ is defined as
    \begin{align}\label{eq:instance-ada2-dz-mu}
    	\mu_{B}((\alpha,\beta))=\frac{1}{2}\left(\nu_{B}((\alpha,0_{d-d_z}))-\|\beta\|_\infty\right).
    \end{align}
    Roughly speaking, our constructions satisfy two properties: for each $j\neq B$ and $1\leq k\leq M_j-1$, 
    \begin{enumerate}
        \item $\mu_{j,k}$ is close to $\mu_B$;
        \item under $I_{j,k}$, pulling an arm that is far from $u_{j,k}$ incurs a regret at least $\frac{r_j}{16}$.
    \end{enumerate}
    The formal version of these two properties are presented in the proof of Lemma \ref{exist_pj-dz} and Lemma \ref{adagrid_lemma-dz}.
    % (1).  (2). }
    % For all arm pulls in all problem instances, an Gaussian noise sampled from $\mathcal{N}(0,1)$ is added to the observed reward. This noise corruption is independent from all other randomness. 
    
    % \textcolor{red}{
    % Let $\mathcal{T}=\{t_1,\cdots,t_B\}$ be any adaptive grid. Our next step is to find an index $j$ such that under world $\mathcal{I}_j$, the batch $(t_{j-1},t_j]$ is sufficiently large. 
    Based on these constructions, we first show that for any adaptive grid $ \mathcal{T} = \{t_0,\cdots,t_B\} $, there exists an index $j$ such that $(t_{j-1},t_j]$ is sufficiently large in world $\mathcal{I}_j$. More formally, for each $j\in[B]$, and event $A_j=\{t_{j-1}<T_{j-1},\;t_j\geq T_j\}$, we define the quantities $p_j := \frac{1}{M_j-1}\sum_{k=1}^{M_j-1}\Pr_{j,k}(A_j)$ for $j\leq B-1$ and $p_B := \Pr_B(A_B)$,
    % quantities $p_j := \frac{1}{M_j-1}\sum_{k=1}^{M_j-1}\Pr_{j,k}(A_j)$ for $j\leq B-1$ and $p_B := \Pr_B(A_B)$,
    where $\Pr_{j,k}(A_j)$ denotes the probability of the event $A_j$ under instance $I_{j,k}$ and policy $\pi$. For these quantities, we have the following lemma.

\begin{lemma}
    \label{exist_pj-dz} 
    For any adaptive grid $\mathcal{T}$ and policy $\pi$, it holds that $\sum_{j=1}^B p_j\geq\frac{7}{8}.$  
\end{lemma} 

\begin{proof}
    For $1\leq j\leq B-1$ and $1\leq k\leq M_j-1$, we write $u_{j,k}=(\hat{u}_{j,k},0_{d-d_z})$. We define $H_{j,k}=\B_{d_z}(\hat{u}_{j,k},\frac{3}{8}r_j)\times[0,1]^{d-d_z}$, where $\B_{d_z}(\hat{u}_{j,k},\frac{3}{8}r_j)$ denotes the $d_z$-dimensional ball with center $\hat{u}_{j,k} $ and radius $ \frac{3}{8}r_j $. It is easy to verify the following properties of our construction (\ref{eq:instance-ada1-dz-nu}), (\ref{eq:instance-ada1-dz-mu}), (\ref{eq:instance-ada2-dz-nu}) and (\ref{eq:instance-ada2-dz-mu}):
    \begin{enumerate}
    	\item $\mu_{j,k}(z)=\mu_B (z)$ for any $z\notin H_{j,k}$;
    	\item $\mu_B (z) \leq \mu_{j,k}(z)\leq\mu_B (z)+\frac{r_j}{8}$, for any $z\in H_{j,k}$.
    \end{enumerate}
    Let $ x_t $ denote the choices of policy $\pi$ at time $t$, and $y_t$ denote the reward. For $t_{j-1}<t\leq t_j$, we define $\Pr_{j,k}^t$ (resp. $\Pr_{B}^{t}$) as the distribution of sequence $\left(x_1,y_1,\cdots,x_{t_{j-1}},y_{t_{j-1}}\right)$ under instance $I_{j,k}$ (resp. $I_B$) and policy $\pi$. Since event $A_j$ can be completely described by the observations up to time $T_{j-1}$ ($A_j$ is an event in the $\sigma$-algebra where $\Pr_{j,k}^{T_{j-1}}$ and $\Pr_B^{T_{j-1}}$ are defined on), we can use the definition of total variation to get 
    \begin{align*}
    	|\Pr_B (A_j)-\Pr_{j,k}(A_j)| 
            =& \;  
            | \Pr_B^{T_{j-1}} (A_j) - \Pr_{j,k}^{T_{j-1}} (A_j) | \\
    	\leq&\;  
            TV \(\Pr_B^{T_{j-1}},\Pr_{j,k}^{T_{j-1}} \) . 
    \end{align*}
    	
    	
    For the total variation, we apply Lemma \ref{lem:pinsker-type} to get 
    \begin{align*} 
    	& \; \frac{1}{M_j-1} \sum_{k=1}^{M_j-1} TV \( \Pr_B^{T_{j-1}},\Pr_{j,k}^{T_{j-1}}\) \\
    	\leq& \; 
    	\frac{1}{M_j-1} \sum_{k=1}^{M_j-1} \sqrt{1-\exp\(-D_{KL}\(\Pr_B^{T_{j-1}}\|\Pr_{j,k}^{T_{j-1}}\)\)}. 
    % 	\label{eq:tv-ada}
    \end{align*} 
    An argument similar to (\ref{chain}) yields that
    \begin{align*}
    	D_{KL}\(\Pr_B^{T_{j-1}}\|\Pr_{j,k}^{T_{j-1}} \) \le \frac{r_j^2}{128} \E_{\Pr_B}\tau_k, 
    % 	\label{eq:chain-rule-ada}
    \end{align*}
    where $\tau_k$ denotes the number of pulls which is in $S_{j,k}$ before the batch containing $T_{j-1}$. Combining the above two inequalities gives
    \begin{align} 
    	& \; \frac{1}{M_j-1} \sum_{k=1}^{M_j-1} TV \( \Pr_B^{T_{j-1}},\Pr_{j,k}^{T_{j-1}}\) \nonumber\\
    	\leq& \;  
    	\frac{1}{M_j-1} \sum_{k=1}^{M_j-1}\sqrt{1- \exp\(-\frac{r_j^2}{128} \E_{\Pr_B}\tau_k\)} \nonumber \\ 
    	\leq& \;  
    	\sqrt{1-\exp\(-\frac{r_j^2}{128(M_j-1)}\E_{\Pr_B}\[\sum_{k=1}^{M_j-1}\tau_k\]\)} \label{l7_jenson-dz} \\ 
    	\leq& \;  
    	\sqrt{  1-\exp\left(-\frac{r_j^2T_{j-1}}{128(M_j-1)}\right)} \label{l7_total-dz} \\ 
    	\leq& \;  
    	\sqrt{ 1-\exp\left(-\frac{1}{64B^2}\right)} \label{l7_useeq-dz} \\ 
    	\leq& \;  \frac{1}{8B}, \nonumber 
    \end{align}
    where (\ref{l7_jenson-dz}) uses Jensen's inequality, (\ref{l7_total-dz}) uses the fact that $\sum_{k=1}^{M_j-1} \tau_k\leq T_{j-1}$, and (\ref{l7_useeq-dz}) uses (\ref{eq:rm-relation-dz}).
        
        
    Plugging the above results implies that
    \begin{align*} 
        |\Pr_B(A_j) - p_j| \le \frac{1}{M_j -1 } \sum_{k=1}^{M_j-1} |\Pr_B (A_j)-\Pr_{j,k}(A_j)| \le  \frac{1}{8B}. 
    \end{align*}
    Since $\sum_{j=1}^B \Pr \(  A_j \) \ge \Pr \( \cup_{j=1}^B A_j \) = 1 $, it holds that 
    \begin{equation*} 
        \sum_{j=1}^B p_j \geq \Pr_B (A_M) +\sum_{j=1}^{B-1} \(\Pr_B(A_j)-\frac{1}{8B} \) \geq \frac{7}{8}.\qedhere
    \end{equation*} 
\end{proof}

Lemma \ref{exist_pj-dz} implies that there exists some $j$ such that $p_j>\frac{7}{8B}$. Then similar to Theorem \ref{thm:lower-static-dz}, we show that the worst-case regret of the policy in world $\mathcal{I}_j$ gives the lower bound we need. 

% Next we proceed with the case where $p_j > \frac{7}{8B}$ for some $j \le B-1$. The case for $j = B$ can be proved analogously. We construct a series of instances
% In world $\mathcal{I}_j$, we use similar method to Theorem \ref{st_lb} to construct a series of instance sets that are difficult to differentiate. More precisely, for any $1\leq k \leq M_j-1$, we construct a set of problem instances $\mathcal{I}_{j,k} = \left(I_{j,k,l} \right)_{1\leq l\leq M_j}$ based on the constructions in (\ref{eq:instance-ada1}) and (\ref{eq:instance-ada2}). For $l\neq k$, the expected reward of $I_{j,k,l}$ is defined as
% \begin{align*}
% 	\mu_{j,k,l}(x)=\left\{
% 	    \begin{aligned}
% 		&\mu_{j,k}(x)+\frac{3r_j}{16},&x=u_{j,l},\\
% 		&\mu_{j,k}(x), & x \in \mathcal{U}_j \; \; \text{ and } \; \; x \neq u_{j,l} , \\ 
% 		&\max\left\{\frac{r_1}{2},\max_{u\in\mathcal{U}_j}\left\{\mu_{j,k,l}(u)-d_{\mathcal{A}}(x,u)\right\}\right\},&otherwise.
% 	\end{aligned}\right.
% \end{align*}
% For $l=k$, we let $\mu_{j,k,k}=\mu_{j,k}$ where $\mu_{j,k}$ is defined as in (\ref{eq:instance-ada1}). For all arm pulls in all problem instances, an Gaussian noise sampled from $\mathcal{N}(0,1)$ is added to the observed reward. This noise corruption is independent from all other randomness. Based on this construction, the following lemma gives the lower bound of expected regret, whose proof is in the Appendix. 
\begin{lemma}\label{adagrid_lemma-dz}
    For adaptive grid $\mathcal{T}$ and policy $\pi$, if index $j$ satisfies $p_j\geq\frac{7}{8B}$, then 
    % (\textcolor{red}{ZF: Is $j$ defined for a fixed $\pi$}?) 
    there exists a problem instance $I$ with zooming dimension $d_z$ such that
    \begin{align*} 
        \E \left[ R_T(\pi) \right] 
        \geq \frac{1}{512B^2}T^{\frac{1-\frac{1}{d_z+2}}{1-\left(\frac{1}{d_z+2}\right)^B}}.
    \end{align*}
\end{lemma}

\begin{proof}
   Here we proceed with the case where $j \le B-1$. The case for $j = B$ can be proved analogously. 
   
   For any $1\leq k \leq M_j-1$, we construct a set of problem instances $\mathcal{I}_{j,k} = \left(I_{j,k,l} \right)_{1\leq l\leq M_j}$.
%   Recall arm set $\mathcal{U}_j=\{u_{j,1},\cdots,u_{j,M_j}\}$ satisfies (a) $d_{\mathcal{A}}(u_{j,m},u_{j,n})\geq r_j$ for any $m\neq n$, and (b) $u_{1,M_1}=\cdots=u_{B,M_B}$. Let $\mu_{j,k}$ be defined as in (\ref{eq:instance-ada1}) . We construct problems instances $I_{j,k,l}$ so that, 
    For $l\neq k$, we first define a function $\nu_{j,k,l}$ on $\A_{d_z}$ as
    \begin{align*}
    	\nu_{j,k,l}(z)
            =
    	    \begin{cases}
    		\nu_{j,k}(z)+\frac{3r_j}{16},\;\text{if}\;z=u_{j,l},\\
    		\nu_{j,k}(z),\;\text{if}\;z\in \mathcal{U}_j\;\text{and}\;  z \neq u_{j,l} , \\ 
    		\max\left\{\frac{r_1}{2},\max_{u\in\mathcal{U}_j}\left\{\nu_{j,k,l}(u)-d_{\mathcal{A}}(z,u)\right\}\right\},\\
            \quad\text{if}\;z\in\A_{d_z}\setminus\mathcal{U}_j,
    	\end{cases}
    \end{align*} 
    where $\nu_{j,k}$ is defined in (\ref{eq:instance-ada1-dz-nu}). Then the expected reward of $I_{j,k,l}$ is defined as 
    \begin{align}\label{eq:instance-ada-jkl-dz-mu}
        \mu_{j,k,l}((\alpha,\beta))=\frac{1}{2}\left(\nu_{j,k,l}((\alpha,0_{d-d_z}))-\|\beta\|_\infty\right),
    \end{align}
    where $(\alpha,\beta)$ is the concatenation of $\alpha\in[0,1]^{d_z}$ and $\beta\in[0,1]^{d-d_z}$. For $l=k$, we let $\mu_{j,k,k}=\mu_{j,k}$. 

    We first show that each $\mu_{j,k,l}$ is $1$-Lipschitz and the zooming dimension equals to $d_z$.
    
    Firstly, for any $(\alpha_1,\beta_1)$ and $(\alpha_2,\beta_2)$, we have
    \begin{align*}
        &\mu_{j,k,l}((\alpha_1,\beta_1))-\mu_{j,k,l}((\alpha_2,\beta_2))\\
        \leq&\mu_{j,k,l}((\alpha_1,\beta_1))-\mu_{j,k,l}((\alpha_1,\beta_2))\\
        &+\mu_{j,k,l}((\alpha_1,\beta_2))-\mu_{j,k,l}((\alpha_2,\beta_2))\\
        \leq&\frac{1}{2}\|\beta_1-\beta_2\|_\infty\\
        &+\frac{1}{2}\big(\nu_{j,k,l}((\alpha_1,0_{d-d_z}))-\nu_{j,k,l}((\alpha_2,0_{d-d_z}))\big)\\
        \leq&\frac{1}{2}(\|\beta_1-\beta_2\|_\infty+\|\alpha_1-\alpha_2\|_\infty)\\
        \leq&\|(\alpha_1-\alpha_2,\beta_1-\beta_2)\|_\infty.
    \end{align*}
    Therefore, $\mu_{j,k,l}$ is $1$-Lipschitz.

    Secondly, for any $r\geq r_j$, (\ref{eq:instance-ada1-dz-mu}) and (\ref{eq:instance-ada-jkl-dz-mu}) yield that $S(16r)\subset[0,1]^{d_z}\times[0, 32r]^{d-d_z}$ and $S(16r)\supset[0,1]^{d_z}\times[0, 30r]^{d-d_z}$. Therefore, we have $30^{d-d_z}r^{-d_z}\leq N_r\leq32^{d-d_z}r^{-d_z}$, and the zooming dimension equals to $d_z$.


    
    Then we show that an argument similar to Lemma \ref{adagrid_lemma} yields the lower bound we need. For each $1\leq k\leq M_j$, we write $u_{j,k}=(\hat{u}_{j,k},0_{d-d_z})$. We define $C_{j,k}= \B_{d_z} \(\hat{u}_{j,k},\frac{r_j}{4} \)\times[0,1]^{d-d_z}$, and our construction $\mathcal{I}_{j,k}$ has the following properties:
    \begin{enumerate}
        \item For any $l\neq k$, $\mu_{j,k,l}(z)=\mu_{j,k,k}(z)$ for any $z\notin C_{j,l}$;
        \item For any $l\neq k$, $\mu_{j,k,k}(z)\leq\mu_{j,k,l}(z)\leq\mu_{j,k,k}(z)+\frac{3r_j}{16}$ for any $z\in C_{j,l}$;
        \item For any $1\leq l\leq M_j$, under $I_{j,k,l}$, pulling an arm that is not in $C_{j,l}$ incurs a regret at least $\frac{r_j}{32}$.
    \end{enumerate}
    Let $x_t$ denote the choices of policy $\pi$ at time $t$, and $y_t$ denote the reward. For $t_{j-1}<t\leq t_j$, we define $\Pr_{j,k,l}^t$ as the distribution of sequence $\left(x_1,y_1,\cdots,x_{t_{j-1}},y_{t_{j-1}}\right)$ under instance $I_{i,j,k}$ and policy $\pi$. From similar argument in (\ref{eq:spl}), it holds that
    \begin{align}
        \sup_{I\in\mathcal{I}_{j,k}}\E \[ R_T(\pi) \] 
        \geq
        \frac{r_j}{32} \sum_{t=1}^T \frac{1}{M_j} \sum_{l=1}^{M_j} \Pr_{j,k,l}^t (x_t\notin C_{j,l}). \label{eq:lower-bound-ada1-dz} 
    \end{align}
    From our construction, it is easy to see that $C_{j,k_1}\cap C_{j,k_2}=\varnothing$ for any $k_1\neq k_2$, so we can construct a test $\Psi$ such that $x_t\notin C_{j,k}$ implies $\Psi\neq k$ . By Lemma \ref{lem:test-tree} with a star graph on $[K]$ with center $k$, we have 
    \begin{align}
        \frac{1}{M_j} \sum_{l=1}^{M_j} \Pr_{j,k,l}^t(x_t\notin C_{j,l}) 
        \ge 
        \frac{1}{ M_j } \sum_{ l \neq k } \int \min \left\{d \Pr_{j,k,k}^t,d \Pr_{j,k,l}^t\right\} . \label{eq:lower-bound-ada2-dz}
    \end{align} 
    
    Combining (\ref{eq:lower-bound-ada1-dz}) and (\ref{eq:lower-bound-ada2-dz}) gives
    \begin{align}
        & \; \sup_{I\in\mathcal{I}_{j,k}} \E \[ R_T(\pi) \] \nonumber \\
        \geq& \;  
        \frac{r_j}{32} \sum_{t=1}^T \frac{1}{M_j}\sum_{l\neq k}\int \min \left\{d \Pr_{j,k,k}^t,d \Pr_{j,k,l}^t\right\}\nonumber  \\ 
        \geq& \; 
        \frac{r_j}{32}\sum_{t=1}^{T_j}\frac{1}{M_j}\sum_{l\neq k}\int\min\left\{d \Pr_{j,k,k}^t,d \Pr_{j,k,l}^t\right\}\nonumber \\
        \geq& \;  
        \frac{r_jT_j}{32}\cdot\frac{1}{M_j}\sum_{l\neq k}\int\min\left\{d \Pr_{j,k,k}^{T_j},  d\Pr_{j,k,l}^{T_j}\right\}\label{eq:lower_cons_1_1-dz} \\ 
        \geq& \;  
        \frac{r_jT_j}{32}\cdot\frac{1}{M_j}\sum_{l\neq k}\int_{A_j}\min\left\{ d \Pr_{j,k,k}^{T_j}, d \Pr_{j,k,l}^{T_j}\right\}\label{eq:lower_cons_1_2-dz} \\ 
        \geq& \;  
        \frac{r_jT_j}{32}\cdot\frac{1}{M_j}\sum_{l\neq k}\int_{A_j}\min\left\{ d \Pr_{j,k,k}^{T_{j-1}}, d \Pr_{j,k,l}^{T_{j-1}}\right\}, \label{eq:lower_cons_1-dz}
    \end{align}  
    where (\ref{eq:lower_cons_1_1-dz}) follows from data processing inequality of total variation and the equation $\int\min\left\{dP,dQ\right\}=1-TV(P,Q)$, (\ref{eq:lower_cons_1_2-dz}) restricts the integration to event $A_j$, and (\ref{eq:lower_cons_1-dz}) holds because the observations at time $T_j$ are the same as those at time $T_{j-1}$ under event $A_j$.
    
    For the term $\int_{A_j}\min\left\{d\Pr_{j,k,k}^{T_{j-1}},d\Pr_{j,k,l}^{T_{j-1}}\right\}$, it holds that 
    \begin{align}
        & \; \int_{A_j}\min\left\{d\Pr_{j,k,k}^{T_{j-1}},d\Pr_{j,k,l}^{T_{j-1}}\right\} \nonumber \\ 
        =&\; \int_{A_j}\frac{d\Pr_{j,k,k}^{T_{j-1}}+d\Pr_{j,k,l}^{T_{j-1}}-\left|d\Pr_{j,k,k}^{T_{j-1}}-d\Pr_{j,k,l}^{T_{j-1}}\right|}{2}\nonumber\\ 
        =&\; 
        \frac{\Pr_{j,k,k}^{T_{j-1}}(A_j)+\Pr_{j,k,l}^{T_{j-1}}(A_j)}{2}-\frac{1}{2}\int_{A_j}\left|d\Pr_{j,k,k}^{T_{j-1}}-d\Pr_{j,k,l}^{T_{j-1}}\right|\nonumber\\
        \geq&\;  
        \(\Pr_{j,k,k}^{T_{j-1}}(A_j)-\frac{1}{2}TV \(\Pr_{j,k,k}^{T_{j-1}},\Pr_{j,k,l}^{T_{j-1}}\)\) \nonumber \\\
        &-TV \(\Pr_{j,k,k}^{T_{j-1}},\Pr_{j,k,l}^{T_{j-1}}\)\label{eq:lower_cons_2_1-dz}\\ 
        =&\; 
        \Pr_{j,k}(A_j)-\frac{3}{2}TV \( \Pr_{j,k,k}^{T_{j-1}},\Pr_{j,k,l}^{T_{j-1}} \), \label{eq:lower_cons_2-dz} 
    \end{align} 
    where (\ref{eq:lower_cons_2_1-dz}) uses the inequality $|\Pr(A)-\mathbb{Q}(A)|\leq TV(\Pr,\mathbb{Q})$, and (\ref{eq:lower_cons_2-dz}) holds because $I_{j,k}=I_{j,k,k}$ and $A_j$ can be determined by the observations up to $T_{j-1}$.
    
    We use an argument similar to (\ref{chain}) to get 
    \begin{align*}
    	D_{KL}\(\Pr_{j,k,k}^{T_{j-1}}\|\Pr_{j,k,l}^{T_{j-1}}\)
    	\le
    	\frac{1}{2}\cdot\left(\frac{3r_j}{16}\right)^2\E_{\Pr_{j,k}}\tau_l
    	\le \frac{r_j^2}{32} \E_{\Pr_{j,k}}\tau_l,
    \end{align*}
    where $\tau_l$ denotes the number of pulls which is in $C_{j,l}$ before the batch of time $T_{j-1}$. Then from Lemma \ref{lem:pinsker-type}, we have
    \begin{align}
        & \; \frac{1}{M_j}\sum_{l\neq k} TV \( \Pr_{j,k,k}^{T_{j-1}},\Pr_{j,k,l}^{T_{j-1}}\) \nonumber \\
        \leq& \; 
        \frac{1}{M_j}\sum_{l\neq k}\sqrt{1-\exp\(-D_{KL}\(\Pr_{j,k,k}^{T_{j-1}}\|\Pr_{j,k,l}^{T_{j-1}}\)\)} \nonumber\\ 
        \leq& \; 
        \frac{1}{M_j}\sum_{l\neq  k}\sqrt{1-\exp\(-\frac{r_j^2}{32}\E_{\Pr_{j,k}}\tau_l\)} \nonumber\\ 
        \leq& \; 
        \frac{M_j-1}{M_j}\sqrt{1-\exp\(-\frac{r_j^2}{32(M_j-1)}\sum_{l\neq k}\E_{\Pr_{j,k}}\tau_l\)} \nonumber\\ 
        \leq& \; 
        \frac{M_j-1}{M_j}\sqrt{1-\exp\(-\frac{r_j^2 T_{j-1}}{32(M_j-1)}\)} \nonumber\\
        \leq& \; 
        \frac{M_j-1}{M_j}\sqrt{1-\exp\(-\frac{M_j}{32(M_j-1) B^2}\)} \label{eq:lower_cons_3_1-dz}\\
        \leq& \; 
        \frac{M_j-1}{M_j}\sqrt{\frac{M_j}{32(M_j-1) B^2}}\nonumber\\
        \leq& \; 
        \frac{1}{4B},\label{eq:lower_cons_3-dz} 
    \end{align}
    where (\ref{eq:lower_cons_3_1-dz}) uses (\ref{eq:rm-relation-dz}).
         
    Combining (\ref{eq:lower_cons_1-dz}), (\ref{eq:lower_cons_2-dz}) and  (\ref{eq:lower_cons_3-dz}) yields that
    \begin{align*} 
        \sup_{I\in\mathcal{I}_{j,k}}\E \[R_T(\pi) \] 
        &\geq 
        \frac{1}{32}  r_jT_j\(\frac{\Pr_{j,k}(A_j)}{2}-\frac{3}{8B}\)\\ &\geq 
        \frac{1}{32B} T^{\frac{1-\varepsilon}{1 -  \varepsilon^B}}\(\frac{\Pr_{j,k}(A_j)}{2} -  \frac{3}{8B}\),
    \end{align*}  
    where $\varepsilon=\frac{1}{d_z+2}$. This inequality holds for any $k \leq M_j-1$. Averaging over $k$ yields
    \begin{align*}
        \begin{split}
            & \; \sup_{I\in\cup_{k\leq M_j-1}\mathcal{I}_{j,k}}\E \[ R_T(\pi) \] \\
            \geq& \; 
            \frac{1}{32B} T^{\frac{1-\varepsilon}{1-\varepsilon^B}} \( \frac{1}{2(M_j-1)}\sum_{k=1}^{M_j-1} \Pr_{j,k}(A_j)-\frac{3}{8B} \)\\ 
            \geq& \; 
            \frac{1}{32B} T^{\frac{1-\varepsilon}{1-\varepsilon^B}} \( \frac{7}{16B}-\frac{3}{8B} \)\\ 
            \geq& \;  
            \frac{1}{512B^2}T^{\frac{1-\varepsilon}{1-\varepsilon^B}}, 
        \end{split}
    \end{align*}
    where the second inequality holds from $p_j\geq\frac{7}{8B}$. Hence, the proof of Lemma \ref{adagrid_lemma-dz} is completed.
\end{proof}

Finally, combining the above two lemmas, we arrive at the lower bound in Theorem \ref{thm:lower-adaptive-dz}.
\end{proof}

==> tex/name.tex <==
For $l=k$, we let $\mu_{j,k,k}=\mu_{j,k}$ where $\mu_{j,k}$ is defined as in (\ref{eq:instance-ada1}). For all arm pulls in all problem instances, an Gaussian noise sampled from $\mathcal{N}(0,1)$ is added to the observed reward. This noise corruption is independent from all other randomness. Based on this construction, the following lemma gives the lower bound of expected regret, whose proof is in the Appendix. 
\begin{lemma}\label{adagrid_lemma}
    For any adaptive grid $\mathcal{T}$ and policy $\pi$, if index $j$ satisfies $p_j\geq\frac{7}{8B}$, then 
    % (\textcolor{red}{ZF: Is $j$ defined for a fixed $\pi$}?) 
    there exists a problem instance $I\in\cup_{k\leq M_j-1}\mathcal{I}_{j,k}$ such that 
    \begin{align*} 
    	\E \left[ R_T(\pi) \right]
    	\geq \frac{1}{256B^2}T^{\frac{1-\varepsilon}{1-\varepsilon^B}}.
    \end{align*}
\end{lemma}

% Finally, similar argument to Theorem \ref{st_lb} yields that
% \begin{align*}
%     \E \left[ R_T(\pi) \right]
%     \geq \frac{1}{256\cdot512^\frac{1}{1-\frac{1}{d+2}}}\frac{1}{B^2}(\log T)^{-\frac{\frac{1}{d+2}}{1-\left(\frac{1}{d+2}\right)^B}}R_z(T)^{\frac{1}{1-\left(\frac{1}{d+2}\right)^B}}.
% \end{align*}
Since $N_r\leq r^{-d}$ holds for all instances, 
\begin{align*}
    \sum_{r=2^{-i},\; r\geq r_0}\frac{N_r}{r}\log T\leq2r_0^{-d-1}\log T.
\end{align*} 
Then we have
% \begin{align*}
% 	R_z(T)=&\inf_{r_0}16r_0T+256\sum_{r=2^{-i},\;r\geq r_0}\frac{N_r}{r}\log T\\
% 	\leq&
% 	\inf_{r_0}16r_0T+512\frac{1}{r_0^{d+1}}\log T\\
% 	=&
% 	16\cdot\left(32\log T\right)^{\frac{1}{d+2}}T^{1-\frac{1}{d+2}}\\
% 	\leq&
% 	512(\log T)^{\frac{1}{d+2}}T^{1-\frac{1}{d+2}}.
% \end{align*}
\begin{align*}
    R_z(T)\leq\inf_{r_0}\left\{16r_0T+512\frac{1}{r_0^{d+1}}\log T\right\}\leq512(\log T)^{\frac{1}{d+2}}T^{1-\frac{1}{d+2}}.
\end{align*}
Consequently, for any policy $\pi$ and adaptive grid $\mathcal{T}$, Lemma \ref{exist_pj}, Lemma \ref{adagrid_lemma} and the above inequality shows that there exists an instance $I$ such that
\begin{align*}
    \E \left[ R_T(\pi) \right]
    &\geq \frac{1}{256B^2}T^{\frac{1-\frac{1}{d+2}}{1-\left(\frac{1}{d+2}\right)^B}}\\ &\geq \frac{1}{256\cdot512^\frac{1}{1-\frac{1}{d+2}}}\frac{1}{B^2}(\log T)^{-\frac{\frac{1}{d+2}}{1-\left(\frac{1}{d+2}\right)^B}}R_z(T)^{\frac{1}{1-\left(\frac{1}{d+2}\right)^B}},
\end{align*}
which concludes the proof.
